Digital Wellbeing Redefined: Toward User-Centric Approach for Positive Social Media Engagement

The prevalence of social media and its escalating impact on mental health has highlighted the need for effective digital wellbeing strategies. Current digital wellbeing interventions have primarily focused on reducing screen time and social media use, often neglecting the potential benefits of these platforms. This paper introduces a new perspective centered around empowering positive social media experiences, instead of limiting users with restrictive rules. In line with this perspective, we lay out the key requirements that should be considered in future work, aiming to spark a dialogue in this emerging area. We further present our initial effort to address these requirements with PauseNow, an innovative digital wellbeing intervention designed to align users' digital behaviors with their intentions. PauseNow leverages digital nudging and intention-aware recommendations to gently guide users back to their original intentions when they "get lost" during their digital usage, promoting a more mindful use of social media.

==> related_work.tex <==
\section{Related Work}
\label{sec:related}

